Knowledge Graph Fusion for Language Model Fine-tuning

Language Models such as BERT have grown in popularity due to their ability to be pre-trained and perform robustly on a wide range of Natural Language Processing tasks. Often seen as an evolution over traditional word embedding techniques, they can produce semantic representations of text, useful for tasks such as semantic similarity. However, state-of-the-art models often have high computational requirements and lack global context or domain knowledge which is required for complete language understanding. To address these limitations, we investigate the benefits of knowledge incorporation into the fine-tuning stages of BERT. An existing K-BERT model, which enriches sentences with triplets from a Knowledge Graph, is adapted for the English language and extended to inject contextually relevant information into sentences. As a side-effect, changes made to K-BERT for accommodating the English language also extend to other word-based languages. Experiments conducted indicate that injected knowledge introduces noise. We see statistically significant improvements for knowledge-driven tasks when this noise is minimised. We show evidence that, given the appropriate task, modest injection with relevant, high-quality knowledge is most performant.

==> [ISCMI] Knowledge Graph Fusion for Language Model Fine-tuning/Chapters/introduction.tex <==
\section{Introduction}
One major challenge in Natural Language Processing (NLP) is assessing the semantic similarity between pairs of text. Since natural language is versatile and ambiguous, it makes rule-based methods difficult to define~\cite{Marsi2013, standfordtyped, schuster-manning-2016-enhanced}. For instance, even though there may be a large discrepancy between the vocabulary used between two text sequences, they can have an equivalent meaning. This discrepancy is due to the polysemous property of most words and the use of synonyms, abbreviations, etc. The converse is also true: text sequences may have similar vocabulary but convey very different meanings, which is often caused by negations and, again, polysemy~\cite{homonymypoly}. Additionally, for domain-specific fields such as sports or medicine, knowledge of the underlying concepts is critical to computing accurate similarity measures~\cite{medicaldomain,oni2020comparative,manaka2022using}.

Humans typically rely on sources of information to fill the gaps in their knowledge. The same concept can be applied to machines. Sources of knowledge such as ontologies, thesauri, and knowledge bases have often been used to improve the performance of various NLP systems~\cite{majavu2008classification,RodriguezWordNet1185844,SemanticTextualSimilarityMethodsToolsAndAppsSurveyarticle}. However, successful integration between the NLP system and knowledge source often requires feature engineering. Furthermore, due to the structural inconsistencies between various knowledge sources, the integration is done in a tightly coupled manner.

The application of pre-trained Language Models for downstream tasks has produced state-of-the-art results in recent years~\cite{kooverjee2020inter,dlamini2019author}. However, the most performant models often contain billions of parameters, requiring expensive computational equipment. It is therefore vital to make such models as efficient as possible, which will also lead to less energy consumption.

Knowledge-Enhanced Models have demonstrated the power of leveraging external knowledge to improve the performance of pre-trained Language Models while retaining model size. The approach by Liu \textit{et al.}\ (2020) \cite{liu2019kbert} combines information from Knowledge Graphs with the ubiquitous BERT model by Delvin \textit{et al.}\ (2018) \cite{devlin-etal-2019-bert} as a means to complement input text with additional domain knowledge or contextual information. Although their results demonstrate benefits for knowledge-driven and domain-specific tasks, the selection mechanism for knowledge injection does not consider sentence context, which may lead to injecting irrelevant or unimportant information. Our study extends K-BERT by modifying the $K_\text{Query}$ mechanism to consider semantically important information and assessing its performance on both open-domain and domain-specific tasks. The utilisation of Wikidata as the Knowledge Graph is done loosely to ensure interchangeability with other knowledge sources. Using ablation studies, we examine the type of knowledge most beneficial to the fine-tuning process and associated limitations. Lastly, since K-BERT was initially developed for the Chinese language, there is a lack of research indicating the level of versatility in the underlying architecture when applied to other languages.

To this end, the article presents the results of our investigation, which show that:
\begin{enumerate}
    \item K-BERT can be successfully adapted to the English domain and possibly other languages.
    \item A modified $K_\text{Query}$ to only inject semantically related information can be beneficial.
    \item Inclusion of external knowledge introduces noise. 
    \item In the absence of noise, external knowledge injection is beneficial to knowledge-driven tasks.
\end{enumerate}

% This paper is organised as follows: Related work will be reviewed in section~\ref{RelatedWork}. Section \ref{KnowledgeGraph} provides details on the Knowledge Graph used and data related preprocessing. Enhancements and changes required to accommodate K-BERT for the English language is detailed in section \ref{Method}. Experiments with ablation studies performed and analysis thereof is discussed in section \ref{Experiment} and \ref{Results} respectively. Final thoughts are concluded in section \ref{Conclusion}, along with suggestions of future work.

